Gradient Descent with Compressed Iterates

We propose and analyze a new type of stochastic first order method: gradient descent with compressed iterates (GDCI). GDCI in each iteration first compresses the current iterate using a lossy randomized compression technique, and subsequently takes a gradient step. This method is a distillation of a key ingredient in the current practice of federated learning, where a model needs to be compressed by a mobile device before it is sent back to a server for aggregation. Our analysis provides a step towards closing the gap between the theory and practice of federated learning, and opens the possibility for many extensions.

==> algs/pgdci.tex <==
\begin{algorithm}[H]
    % \SetAlgoLined
    \caption{Gradient Descent with Compressed Iterates}
    \label{alg:pgdci}
    \begin{algorithmic}[1]
        \REQUIRE{Stepsize $\gamma > 0$  }
        \STATE Initialize $x_0\in \R^d$ \\
        \FOR{$k= 1, 2, 3, \ldots$}
            \STATE Compress the current iterate:
            \begin{equation}
                v_k = \cC(x_k)
            \end{equation}
            \STATE Perform a gradient descent update:
            \begin{equation}
                \label{rgdci-update}
                x_{k+1} = v_k - \gamma \nabla f(v_k)
            \end{equation}
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
